Quarl: A Learning-Based Quantum Circuit Optimizer

Optimizing quantum circuits is challenging due to the very large search space of functionally equivalent circuits and the necessity of applying transformations that temporarily decrease performance to achieve a final performance improvement. This paper presents Quarl, a learning-based quantum circuit optimizer. Applying reinforcement learning (RL) to quantum circuit optimization raises two main challenges: the large and varying action space and the non-uniform state representation. Quarl addresses these issues with a novel neural architecture and RL-training procedure. Our neural architecture decomposes the action space into two parts and leverages graph neural networks in its state representation, both of which are guided by the intuition that optimization decisions can be mostly guided by local reasoning while allowing global circuit-wide reasoning. Our evaluation shows that Quarl significantly outperforms existing circuit optimizers on almost all benchmark circuits. Surprisingly, Quarl can learn to perform rotation merging, a complex, non-local circuit optimization implemented as a separate pass in existing optimizers.

==> motivation.tex <==
\section{The Circuit Optimization Search Space\label{sec:motivation}}
\if 0
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figs/figure1_search_space_dist_v3.pdf}
    \caption{Number of circuits equivalent to \tof in the search space by applying different numbers of transformations.}
    \label{fig:search_space}
\end{figure}
\fi 
%\begin{figure}
%    \centering
%    \includegraphics[scale=0.4]{figs/figure1_connectivity.pdf}
%    \caption{Search space}
%    \label{fig:connecitivy}
%\end{figure}

\begin{figure}
    \centering
    \subfloat[\tof]{
    \includegraphics[scale=0.45]{figs/seq_barenco_tof_3.pdf}
    }
    \\
    \subfloat[{\tt seq\_qcla\_com\_7}]{
    \includegraphics[scale=0.45]{figs/seq_qcla_com_7.pdf}
    }
    \caption{Caption}
    \label{fig:sequence_analysis}
\end{figure}

This section analyzes long-sequence optimizations, which reduce the cost of quantum circuits by applying a {\em long} sequence of transformations while {\em any} subset of these transformations does not \yw{may not?} directly reduce cost.
%%%
We perform a case study on the search space of deploying the \tof circuit~\cite{nam2018automated}, which includes three Toffoli gates  and is represented in the Nam gate set \{$CNOT$, $X$, $H$, $T$, $T^\dag$\}. A Toffoli gate provides an implementation of the universal reversible gate and is a key building block of modern quantum algorithms.
%of the quantum circuit \tof~\cite{nam2018automated}, which includes three Toffoli gates and was introduced by Barenco et al.~\cite{Barenco_1995}.\ZL{what's the application of it?}.
%Our observations can generalize to quantum circuits for various applications.
%and acknowledge that our observations and analyses on \tof generalize to other quantum circuits.
%%%
To optimize the \tof circuit, we consider the 8668 circuit transformations discovered by Quartz~\cite{pldi2022-quartz} for the Nam gate set.
We identify three key challenges of discovering long-sequence optimizations.

%This section analyzes long-sequence optimizations by identifying three key challenges we must address in order to discover them to optimize quantum circuits on NISQ devices.
%\ZJ{Say that the experiments were conducted on the barenco circuit }

\paragraph{Large search space.}

Given an input circuit and a set of transformations, our search space is composed of all circuits reachable from the input circuit by applying the transformations. These circuits are all equivalent to the input circuit, and we are looking for an optimal one according to some cost functions. A naive exhaustive search approach is not practical except for very small circuits, since the number of equivalent circuits that are reachable via transformations is much to large for exhaustive exploration. For example, some transformations allow to swap two gates; if a circuit contains 100 pairs of swappable gates, there are at least $2^100$ equivalent circuits. In practice, transformations do much more than just swapping gates, so the search space of equivalent circuits is both very large and not clearly structured or unifrom.

\paragraph{Large search space.} The first challenge of optimizing quantum circuits is to deal with the extremely large search space associated with each circuit.
Specifically, for an input circuit, iteratively applying transformations on the circuit results in many circuits functionally equivalent to the original one, constituting a large and complex search space. 
%%%%
\Cref{fig:search_space} shows the number of equivalent circuits in the search space by applying different numbers of transformations on \tof. 
The search space size grows 

exponentially in the number of transformations applied.
As a result, discovering long-sequence optimizations requires exploring large search spaces with billions of candidate circuits.

\paragraph{Planar optimization landscape.}
Despite the extremely large search space, the second challenge of discovering long-sequence optimizations is dealing with the planar optimization landscape associated with each circuit in the search space.
%%%
To characterize this challenge, we sample a thousand circuits from the search space shown in \Cref{fig:search_space} and measure the {\em minimal} number of transformations we have to apply to reduce a circuit's cost. 
%%%
For each sampled circuit $C$, we perform a breadth-first-search (BFS) to apply transformations and terminate the search when a circuit $C'$ with lower cost is discovered.
%%%
Therefore, the number of transformations applied to obtain $C'$ indicates the radius of the planar optimization landscape associated with $C$, since applying fewer transformations to $C$ cannot reduce its cost.
Figure~\ref{fig:all_dist} shows the result when using the total gate count as the cost metric. For more than half of the sampled circuits, reducing the total gate counts requires applying more than four transformations.
%\ZJ{Analyze the circuit depth results.}

\paragraph{Performance-decreasing transformations.}
The third challenge of discovering long-sequence optimizations is the necessity of using transformations that temporarily decrease performance.
%%%
For example, the first transformation in \Cref{fig:long-sequence} increases the circuit depth from 8 to 9, which is necessary to enable the subsequent transformations that finally reduce the circuit depth to 7.
%%%
For the \tof circuit, without using the performance-decreasing transformations, the best circuit that can be discovered includes 46 gates, while considering the performance-decreasing transformations can further reduce the gate count to 36.

Performance-decreasing transformations are critical to discovering highly optimized circuits in \sys. Figure xxx compares the performance of the best discovered circuits when including and excluding performance-decreasing transformations.
\ZJ{}
However, determining when and where to apply performance-decreasing transformations is non-trivial, since these transformations are only beneficial when combined with other transformations that further improve performance.
%%%

%\ZJ{Say that \sys performs many performance-decreasing transformations in our evaluation.}

\if
\section*{Old Version, to be removed}
\paragraph{Large search space.}
To optimize a quantum circuit, the first challenge we have to address is exploring an extremely large search space of circuits functionally equivalent to the input circuit.
%%%
Specifically, for a quantum circuit, the search space includes all circuits that can be obtained by applying one or multiple transformations on the input circuit.
\Cref{fig:search_space} characters the search space of the {\tt barenco\_tof\_3} circuit, which includes four Toffoli gates and was introduced in~\cite{Barenco_1995}.
%%%
Each bar indicates the number of {\em distinct} circuits that can be obtained by applying a sequence of $k$ transformations generated by Quartz on the original circuit.
%%%
As shown in the figure, the number of circuits reachable from the input circuit grows exponentially.

\paragraph{Planar optimization landscape.}
%Despite the extremely large search space, a second challenge of discovering long-sequence optimizations is dealing with the planar optimization landscape associated with each candidate circuit.
%%%
To assess the optimization landscape of a circuit, we measure the minimal number of transformations we have to apply to reduce its cost.
For each circuit in the search space, we perform a breadth-first-search (BFS) and terminate the search when discovering a circuit with lower cost.
%%%
We observe that the optimization landscapes highly depend on the gate count and categorize the circuits based on their gate counts.

\paragraph{Performance-decreasing transformations.}
A third challenge is the necessity of performance-decreasing transformations, since many long-sequence optimizations involve transformations that increase the circuit cost as intermediate steps, such as the example in \Cref{fig:long-sequence} when using circuit depth as the cost metric.
%%%

\ZJ{To be removed.}
\begin{itemize}
    \item One figure that demonstrate the connectivity between circuits in a search space. May need to sample a subset of circuits.
    \item CDF figures indicating that long-sequence optimizations are prevalent for circuits in the above search space
    \item A figure showing that we may need to apply long-sequence optimizations multiple to find optimized circuits. Maybe some the cases for different input circuits.
\end{itemize}
\fi 
